Efficient Data-Driven MPC for Demand Response of Commercial Buildings

Model predictive control (MPC) has been shown to significantly improve the energy efficiency of buildings while maintaining thermal comfort. Data-driven approaches based on neural networks have been proposed to facilitate system modelling. However, such approaches are generally nonconvex and result in computationally intractable optimization problems. In this work, we design a readily implementable energy management method for small commercial buildings. We then leverage our approach to formulate a real-time demand bidding strategy. We propose a data-driven and mixed-integer convex MPC which is solved via derivative-free optimization given a limited computational time of 5 minutes to respect operational constraints. We consider rooftop unit heating, ventilation, and air conditioning systems with discrete controls to accurately model the operation of most commercial buildings. Our approach uses an input convex recurrent neural network to model the thermal dynamics. We apply our approach in several demand response (DR) settings, including a demand bidding, a time-of-use, and a critical peak rebate program. Controller performance is evaluated on a state-of-the-art building simulation. The proposed approach improves thermal comfort while reducing energy consumption and cost through DR participation, when compared to other data-driven approaches or a set-point controller.

==> Section/Annexe.tex <==
\begin{figure*}
\centering     %%% not \center
\subfigure[Zone 1]{\includegraphics[trim=0cm 0.5cm 0cm 0cm, clip,width=90mm]{Figures/fit/Linear_ts_z1.pdf}}\label{subfig:linear_zone1}
\subfigure[Zone 2 ][b]{\includegraphics[trim=0cm 0.5cm 0cm 0cm, clip,width=90mm]{Figures/fit/Linear_ts_z1.pdf}}\label{subfig:linear_zone2}
\subfigure[Zone 1 ]{\includegraphics[trim=0cm 0.5cm 0cm 0cm, clip,width=90mm]{Figures/fit/Convex_ts_z1.pdf}}\label{subfig:Convex_zone1}
\subfigure[Zone 2 ]{\includegraphics[trim=0cm 0.5cm 0cm 0cm, clip,width=90mm]{Figures/fit/Convex_ts_z2.pdf}}\label{subfig:Convex_zone2}
\subfigure[Zone 1 ]{\includegraphics[trim=0cm 0.5cm 0cm 0cm, clip,width=90mm]{Figures/fit/lstm_ts_z1.pdf}}\label{subfig:lstm_zone1}
\subfigure[Zone 2 ]{\includegraphics[trim=0cm 0.5cm 0cm 0cm, clip,width=90mm]{Figures/fit/lstm_ts_z2.pdf}}\label{subfig:lstm_zone2}
\caption{\gls{iat} predictions. (a)--(b) linear model. (c)--(d) \gls{icrnn} model. (e)--(f) \gls{lstm} model.}
\label{fig:fit}
\end{figure*}

==> Section/annexe.tex <==
 %\begin{align}
%\underset{\text{$\hat{\mathbf{u}}^{k}$, $p^{k}_{+}$,  $p^{k}_{-}$}}{\text{ min }} &  \sum_{k \in \mathcal{T}} \lambda_{E}E^{k} - \sum_{ k \in \mathcal{T}\setminus \mathcal{W}} \lambda_{+}^{k} E^{k}_{+}  - \sum_{ k \in \mathcal{T}\setminus \mathcal{W}}  \lambda_{-}^{k} E^{k}_{-}   \label{DR_obj} \\  
% \text{  s.t. } \quad  & (\ref{dynamics})-(\ref{c_domain}) \nonumber  \\ 
%& \mathbf{u}^{k}^\top  \mathbf{p}^{c}  - p^{k}_{\text{baseline}} = p^{k}_{+} - p^{k}_{-}, \quad \forall k \in \mathcal{T}\setminus \mathcal{W} \label{p_bid} \\ 
%& p^{k}_{+} \geq 0, \quad  p^{k}_{-} \geq 0, \quad \forall k \in \mathcal{T}\setminus \mathcal{W} \label{bid_domain} \\ 
%& p^{k}_{+} \leq M(1-z^{k}), \quad  \forall k \in \mathcal{T}\setminus \mathcal{W} \label{disjonctive_c1} \\ 
%& p^{k}_{-} \leq Mz^{k}, \quad  \forall k \in \mathcal{T}\setminus \mathcal{W} \label{disjonctive_c2}  \\  
%& \mathbf{u}^{k}^\top  \mathbf{p}^{c}  - p^{k}_{\text{baseline}} \geq c^{k}_{+},  \text{ if }  \sigma^{k}_{+}=1,  \forall k \in \mathcal{W} \label{bid_up} \\
%& p^{k}_{\text{baseline}} - \mathbf{u}^{k}^\top  \mathbf{p}^{c}  \geq c^{k}_{-},   \text{ if }  \sigma^{k}_{-}=1,  \forall k \in \mathcal{W} \label{bid_down} \\ 
%&  E^{k}_{+/-} =p^{k}_{+/-} \Delta t, \quad \forall k \in \mathcal{T}\setminus \mathcal{W} \label{energy_bid} \\
% & z^{k} \in \{0,1\},  \quad p^{k}_{+}, p^{k}_{-} \in \mathbb{R} \quad \forall k \in \mathcal{T}\setminus \mathcal{W} \label{z_domain}
%\end{align} 

The objective function (\ref{DR_obj}) is expressed in terms of the cost of the energy consumed and a penalty. Howver, when the energy consumed is lower than the baseline, the penalty term is equal as the reward for the services provided. Constraint~(\ref{adjusment}) is the amount of energy adjusment with respect to the baseline. Once a bid is cleared in the market, participants are expected to provide the adequate service when called by the \gls{iso}. This is modeled (\ref{bid_up})$-$(\ref{bid_down}).


%energy Constraints (\ref{p_bid})$-$(\ref{bid_domain}) defines the services of power curtailment $p^{k}_{-}$ or power increase $p^{k}_{+}$ with respect to the baseline consumption. Constraints (\ref{disjonctive_c1})$-$(\ref{disjonctive_c2}) express that the building cannot curtail and increase power at the same time. Once a bid is cleared in the market, participants are expected to provide the adequate service when called by the \gls{iso}. This is modeled (\ref{bid_up})$-$(\ref{bid_down}). (\ref{energy_bid}) is the amount of energy dedicated to the services.  Finally, (\ref{bid_domain})$-$(\ref{z_domain}) describe the domain of the optimization variables.


\subsubsection{Metrics}
$\Vert T(\mathbf{u}^{t}) \Vert_{1}$ is defined as the metrics for measuring \gls{rtu} toggling at a timestep $t$: 
\begin{align*}
    T(\mathbf{u}^{t})=\sum_{\tau=k-\rho}^{k-1} \left( \max\left\{ \mathbf{u}^{\tau-1}-\mathbf{u}^{\tau}\right\}\right) - (1-\mathbf{u}^{t})
\end{align*} 

and discomfort is defined as sum of discomfort across rooms over time. 


==> Trash/Annexe_2.tex <==
Naturaly, the objective would be formulated as the costs of power and reward, $R(\mathbf{u}^{k})=\lambda_{-}^{k}\max\left\{p^{k}_{\text{baseline}}- \mathbf{u}^{k}^\top \mathbf{p}^{c}, 0\right\} \Delta t$, as the reward is obtained only if adjustments are made to be below the baseline. However, to maintain convexity of the optimization problem, we reformulate the reward term as a penalty term. Also, since the problem is solve via-DFO, inequality constraints are easier to formulate. 


\gls{dr} formulation for the linear-based model : 
\begin{align}
\underset{\text{$\hat{\mathbf{u}}^{k}$, $p^{k}_{+}$,  $p^{k}_{-}$}}{\text{ min }} &  \sum_{k \in \mathcal{T}} \lambda_{E}E^{k} - \sum_{ k \in \mathcal{T}\setminus \mathcal{W}} \lambda_{+}^{k} E^{k}_{+}  - \sum_{ k \in \mathcal{T}\setminus \mathcal{W}}  \lambda_{-}^{k} E^{k}_{-}   \label{DR_obj} \\  
 \text{  s.t. } \quad  & (\ref{dynamics})-(\ref{c_domain}) \nonumber  \\ 
& \mathbf{u}^{k}^\top  \mathbf{p}^{c}  - p^{k}_{\text{baseline}} = p^{k}_{+} - p^{k}_{-}, \quad \forall k \in \mathcal{T}\setminus \mathcal{W} \label{p_bid} \\ 
& p^{k}_{+} \geq 0, \quad  p^{k}_{-} \geq 0, \quad \forall k \in \mathcal{T}\setminus \mathcal{W} \label{bid_domain} \\ 
& p^{k}_{+} \leq M(1-z^{k}), \quad  \forall k \in \mathcal{T}\setminus \mathcal{W} \label{disjonctive_c1} \\ 
& p^{k}_{-} \leq Mz^{k}, \quad  \forall k \in \mathcal{T}\setminus \mathcal{W} \label{disjonctive_c2}  \\  
& \mathbf{u}^{k}^\top  \mathbf{p}^{c}  - p^{k}_{\text{baseline}} \geq c^{k}_{+},  \text{ if }  \sigma^{k}_{+}=1,  \forall k \in \mathcal{W} \label{bid_up} \\
& p^{k}_{\text{baseline}} - \mathbf{u}^{k}^\top  \mathbf{p}^{c}  \geq c^{k}_{-},   \text{ if }  \sigma^{k}_{-}=1,  \forall k \in \mathcal{W} \label{bid_down} \\ 
&  E^{k}_{+/-} =p^{k}_{+/-} \Delta t, \quad \forall k \in \mathcal{T}\setminus \mathcal{W} \label{energy_bid} \\
 & z^{k} \in \{0,1\},  \quad p^{k}_{+}, p^{k}_{-} \in \mathbb{R} \quad \forall k \in \mathcal{T}\setminus \mathcal{W} \label{z_domain}
\end{align}   

\gls{dr} formulation for non-convex \gls{mpc}: 

\begin{align}
\underset{\text{$\hat{\mathbf{u}}^{k}$}}{\text{ min }} &  \sum_{k \in \mathcal{T}} \lambda_{E}E^{k}  - \sum_{ k \in \mathcal{T}\setminus \mathcal{W}}\lambda_{-}^{k} \Delta E^{k}_{-} \label{DR_obj} \\  
 \text{  s.t. } \quad  & (\ref{dynamics})-(\ref{c_domain}) \nonumber  \\ 
& \Delta E_{-}^{k}= \left(p^{k}_{\text{baseline}}- \mathbf{u}^{k}^\top  \mathbf{p}^{c}\right)\Delta t \quad \forall k \in \mathcal{T}\setminus \mathcal{W} \label{adjusment} \\   
& p^{k}_{\text{baseline}} - \mathbf{u}^{k}^\top  \mathbf{p}^{c}  \geq c^{k}_{-},   \text{ if }  \sigma^{k}_{-}=1,  \forall k \in \mathcal{W} \label{bid_down}  
\end{align}   




==> Trash/Intro_trash.tex <==
Availabitlity of data and data-driven approaches. 
\begin{itemize}
    \item the advances in Information and  Communication Technology (ICT), decreasing hardware cost, and improving data accessibility, have allowed the collection and storage of a large amount of high-quality building-related data, allowing the development of more accurate and robust data-driven approaches \cite{data_driven_hvac_review}. 
    \item Data-driven approaches promote wide-scale implementation of control strategies as does not require an understanding of the system dynamics, can provide good prediction accuracy if sufficient amount data \cite{HVAC_modelling}.
\end{itemize}

\cite{gonzalez2022review}:
\begin{itemize}
    \item The Built environment is one of the most energy intensive sector and one of the main contributor to climate change 
    \item Buildings accounts for 30\% of the global energy consumption and 28\% of total greenhouse emissions. 
    \item In commercial building \gls{HVAC} systems accounts 47\% of of the building consumption. 
\end{itemize}

\cite{HVAC_modelling}:
\begin{itemize}
    \item Many research have shown that appropriate HVAC operation can provide energy savings while maintaning thermal comfort. 
    \item it has been shown that its more sustainable and costs effective to improve control systems than upgrading HVAC equipment with more modern and efficient HVAC technologies
\end{itemize}

\begin{itemize}
    \item In the US, 90\% are small (5,000 sf) or medium (between 5,000 sf and 50,000 sf) and most of them and rudimentary controller (ruled-based controller)\cite{smb_2012} 
    \item Most small-medium commercial are RTU based. \cite{smb_2012}
    \item Over half of commercial building floor area is served by packaged HVAC %DOE. 2017. Energy savings potential and RD&D opportunities for commercial building HVAC Systems. U.S. Department of Energy.https://www.energy.gov/sites/prod/files/2017/12/f46/bto-DOEComm-HVAC-Report-12-21-17.pdf
\end{itemize}

\begin{itemize}
    \item Modeling buildings can be challenging due to their highly nonlinear nature and presence of large disturbances.The resulting nonlinear optimization problem may have multiple local solutions. Hence a tradoff exists between accuracy and simplicity for optimization \cite{Handbook_MPC}. 
    \item In last years, MPC has demonstrated to be well-suited for BEM applications focused on improving the energy consumption and the users’ comfort, being able to exploit the predictions of future disturbances, such as weather. \cite{data_driven_hvac_review}.
    \item  The main benefit of MPC is a systematic thermal comfort improvement with simultaneous energy savings spanning from 15\% up to 50\% demonstrated on numerous simulation and several pilot case studies \cite{review_MPC}.
    \item The strength of  MPC lies in the use of a mathematical model of the building to predict its future behavior. By using these predictions, MPC can optimally choose the control actions based on a given objective while taking into account the comfort and technological constraints, and weather forecasts in a systematic and flexible way \cite{review_MPC}. 
    \item Despite the abundance of research papers and several pilot installations, the transfer of this technology to the building market is still in its early stages \cite{review_MPC}.
    \item  main challenges for wide-spread application of MPC to buildings are defined: Automated design, tuning, and deployment of MPC. -> Link with data-driven.
    \item Naturally, the quality of the MPC solution relies on the model accuracy, but also the 
overall MPC implementation is affected by the chosen modeling 
approach in a number of ways. Efficient optimization algorithms utilize 
specific model characteristics, like linearity, continuity, or known derivatives. However, the phenomena and processes occurring in buildings 
are often nonlinear and discontinuous, and complex physical models or 
advanced data-driven models are required to model such processes 
accurately. On the other hand, more complex models increase the 
overall computational demand of MPC, not only by increased simulation 
time but also because they are not suitable for efficient optimization 
algorithms and gradient-free algorithms have to be used instead. 
Therefore, a sound trade-off between the model accuracy and simplicity 
is required.
\end{itemize}

Modelling paradigms \cite{review_MPC} \\ 
White-box models 
\begin{itemize}
 \item White-box: White-box models describe the building dynamics from physical knowledge. The main challenge in white-box modeling is the significant effort required to describe the building properties. The resulting model typically  includes hundreds or, more likely, thousands of parameters. Hence,  there are many potential sources of model inaccuracy, making the process of parameter setup difficult.
    \item  If detailed technical documentation and physics-based modeling expertise are available, then it may be preferable to follow the white-box approach, as it leads to reliable and interpretable models with little requirements on the sensor data amount and quality. 
\end{itemize}

Black-box model:
\begin{itemize}
    \item Black-box models learn the dynamics of the buildings from the measured data without making any prior assumptions regarding any physical relationships.  they usually lead to lower development cost. 
    \item On the other hand, if extensive reliable measurement data is available, the black-box approach provides  models which are often more accurate and easily transferable to different buildings and systems, reducing the implementation time
    \item Linear models The simplest and most intuitive black-box models are the parametric linear models  \cite{review_MPC}. 
    \item Pour assurer la \textcolor{red}{l'efficacité de la résolution}, des modèles simples tels que les modèles du premier ordre sont souvent utilisés \cite{BIRD_2022, KIM_2018, KIM2022112118, ZHANG_2017}. Cependant, de tels modèles ont une puissance de modélisation limitée, et la dynamique thermique des bâtiments loin d'être linéaire, ce qui peut entraîner des performances médiocres du contrôleur. 
     \item Artificial Neural Networks (ANN) : However, model predictive control on real commercial buildings is still challenging because it has a complicated structure, which results in non-convex optimization problems that are hard to solve, namely : \cite{BBAI, building_RNN}.
     \item Non-optimization based data-driven method remain impletmented in pratice due to performance, scalability and robustness As a results, predictive control (non-optimization based methods) are more commonly implemented \cite{DPC_2018}, \cite{DENG_2023}.
\end{itemize}

Availabitlity of data and data-driven approaches. 
\begin{itemize}
    \item the advances in Information and  Communication Technology (ICT), decreasing hardware cost, and improving data accessibility, 
have allowed the collection and storage of a large amount of high-quality building-related data, allowing the development of more accurate and robust data-driven approaches \cite{data_driven_hvac_review}. 
    \item Data-driven approaches promote wide-scale implementation of control strategies as does not require an understanding of the system dynamics, can provide good prediction accuracy if sufficient amount data \cite{HVAC_modelling}.
\end{itemize}

Data-driven modeling of modeling of building thermal dynamics~\cite{wang2019data}: 
\begin{itemize}
    \item Building thermal process can be nonlinear 
\end{itemize}

\cite{shaikh2014review}:
\begin{itemize}
    \item  MPC  technology involves huge costs for modeling, data collection, expert monitoring and deployment; due to which, it is not worth-it for medium sized buildings.
\end{itemize}

%buildings' contributions to the power grid balance, enhancing the reliability and making both building and the grid more efficient. 


%\textcolor{red}{intro DR}. :
%\begin{itemize}
%    \item Acheiving real-time control of commercial building is an important step towards grid-responsive building : buildings' contributions to the power grid balance, enhancing the reliability and making both building and the grid more efficient. 
%    \item Proposing a demand response strategy 
%    \item \glspl{cb} are among the largest consummers and controlling effectively their \gls{hvac} systems has the potential to levrage large amount for the grid.  
%    \item By levraging flexibility, its benefits the network and generate additonnal revenu for the building. For the grid its promotes economy and reliability. 
    %\item Controlling the building in real-time (5 minutes) 
    %\item Buildings have a natural source of flexibility through their thermal mass which act as a passive thermal storage. By precooling or preheating zones before DR event, they can participate to DR event while maintaining thermal comfort. 
%\end{itemize}


%Modeling the thermal dynamics of a building can be a challenging task due to its highly nonlinear nature and the presence of larges disturbances~\cite{Handbook_MPC, wang2019data}. Many approaches rely on \glspl{nn} for their high modeling accuracy and ability to account for complex interactions among inputs \cite{wang2019data}. Nevertheless, applying \glspl{nn} to commercial buildings (\glspl{cb}) presents challenges, as it results in non-convex optimization problems that are computationally intractable \cite{BBAI, building_RNN, reynolds2018zone}. As a result, first-order models are often used in practice to ensure computational tractability \cite{BIRD_2022, KIM_2018, KIM2022112118, ZHANG_2017}. Alternatively, non-optimization-based data-driven approaches, such as predictive control, are more commonly implemented in \glspl{cb} \cite{DPC_2018, DENG_2023, huang2015neural}.

%-The quality of the\gls{mpc} solution rely on the quality of model accuracy and the ability to efficiently solve the problem globaly and efficiently~\cite{review_MPC}. 
%-a sound trade-off between the model accuracy and simplicity is required~\cite{review_MPC}. 



%Additionally, they can often achieve higher accuracy when sufficient data is available 
%and their ability to account for complex interactions between inputs


%Modeling a building thermal dynamics can be challenging task due to their highly nonlinear nature~\cite{Handbook_MPC,wang2019data}. Many have based their modelling approach on \glspl{nn} for their high modeling accuracy and abilities to account for complex interaction between inputs\cite{wang2019data}. \glspl{nn}-MPC approaches have been applied on \glspl{cb}~\cite{BBAI, building_RNN, reynolds2018zone}. However, they result in a non-convex optimization problems and are computationnaly intractable. As a results, first-order model remain used in pratice to ensure computational tracktability~\cite{BIRD_2022, KIM_2018, KIM2022112118, ZHANG_2017}, even though they may not fully capture the building dynamics~\cite{wang2019data}. Or non-optimization approaches based data-driven such as predictive control are more commonly implemented~\cite{DPC_2018, DENG_2023, huang2015neural}. 

%hand, \gls{nn} with ReLU activation are piecewise linear \cite{arora2018understanding}, and therefore non-smooth optimization programs.

%The piecewise linear nature has encourage approaches consisting to reformulate the ReLu-based \gls{nn} as the \gls{mip} reformulation has the benefits of producing provably optimal solutions \cite{Anderson_2020,Tsay_2021}. This approach can approach makes integer optimization variables straightforward. However, it has the downside of introduce a large number of binary variable wich can leads to intractabability in the \gls{mpc} context. Also, these is a lack of exact and computational effective reformulation for various \gls{nn} architectures have not yet been developed in the litterature.
%Other approachs based on metaheuristic such as via genetic algorithm have been applied to solve non-convex mixed-integer \cite{BBAI} . In the methods readily available, only \gls{mip} reformulation, some metaheuristics algorithms and some \gls{dfo} algorithms. In this work, we base our approach on the \gls{dfo} mature solver \texttt{NOMAD}. It should be emphasis that a gradient-based approach will always outperform \gls{dfo}, as a results obtained are a lower-bound on the possible performances of the controller. 



%Other have focused on gradient based method exploting the fact that gradients of \gls{nn} can be easily computed via backpropagation, or bundled entropy method. ReLu-based \gls{nn} are non-smooth function, so gradient descent is not garanteed to converge. Moreover. other approaches where based on \gls{dfo}. It should be emphasised that all approaches were considering continous variables. In this work, we base our approach on \gls{dfo}
%\cite{WANG} : Comparison of reinforcement learning and model predictive control for building energy system optimization. The MPC controller is based on a reduced-order thermal resistance-capacity network model. Results showed that the MPC controller is superior to the RL and baseline controller on scenarios on the virtual test bed (Modelica). 

%\begin{itemize}
%\item Optimization-Based Data-Enabled Modeling Technique for HVAC Systems Components: https://doi.org/10.3390/buildings10090163 
%\item https://doi.org/10.1016/j.engappai.2023.106226
%\item https://doi.org/10.1016/j.enbuild.2017.02.012 
%\end{itemize}

==> Trash/Litterature_review_trash.tex <==
%Plan : 
%\begin{itemize}
% item RTU control in commercial buildings : 
%\item classical methods 
%\item Data-driven and non-convex 
%\item Data-driven and convex method 
%\end{itemize}

%Control strategies applied to (\gls{rtu})-\gls{hvac} control \cite{Review_control}

%\begin{itemize}
%    \item \cite{HVAC_modelling} "The ability if data-driven approaches in modeling HVAC system has been established in various research studies" 
%    \item 
%\end{itemize}
 
%MPC has been widly applied to commerical building for centralized \gls{hvac} systems control. Building modelling techniques can be divided into three categories: physics-based, data-driven and gray box \cite{HVAC_modelling}. Most approaches and real-life implementation case-study remain based on simple model/low-order to ensure tractability. In \cite{BIRD_2022}, a real-world case study in a large commercial buildings. The MPC scheme seek to minimise energy cost and use a low-order linear model (ARX model) of the building. Performances of the controller are then assessed in simulation on a RC building thermal model. The proposed MPC improve of 1.7 \% energy saving compared to the PI controller (baseline). In \cite{KIM_2018} : MPC for RTUs of small-medium commercial buildings. The study consider a state-space model-based MPC. The control problem is aiming to determine the trajectory of all RTUs over a short horizon (ex: 30 min , sampling time 5 min) to minimize energy use and peak demand, and deviation from comfort bound. Staging is assumed to be fixed (no cycling). The proposed controller shows 12 \% HVAC energy savings and 18\% HVAC peak demand demand reduction compared with a conventional thermostat during a a real-life 4 month experiment. Article of the same author : \cite{KIM2022112118}. Also, performances are assessed on a limited model of the buildings. \cite{ZHANG_2017} proposed an algorithm to coordinate RTUs of small- and medium-sized commercial buildings. The proposed algorithm is an mixed integer linear program with the objective of minimizing the total cost from occupants discomfort and energy consumption. \\ 
%\textcolor{red}{tractable approaches}

%"Data-driven approaches promote wide-scale implementation of control strategies as does not require an understanding of the system dynamics, can provide good prediction accuracy if sufficient amount data \cite{HVAC_modelling}" "Data-driven approches have demonstrated to overcome the main short commings of physical based methods, since they do not need an in-depth knowledge of the physical problem, avoiding complex mathematical calculations and reducing computational requirements." "In the recent years, the advances in ICT ... have allowed the collection and storage of a large amount of high quality building-related data"\cite{data_driven_hvac_review} 

%\begin{itemize}
%\item \cite{BBAI} : LSTM with attention mechanism based MPC with a genetic algorithm. Non-convex, cannot garantee optimality. (centralized)   
%\item \cite{DENG_2023}: (not MPC) Evaluate effectiveness, robustness and scalability of data-driven predictive control. The experiment was conducted on 78 buildings of the RTEM database and historical data were used to train a deep neural network (DNN) as a building model and was then used to for energy saving. Average energy saving of 65 \% and peak load reduction of 15 \% compared to control. 
%\item Optimization-Based Data-Enabled Modeling Technique for HVAC Systems Components: https://doi.org/10.3390/buildings10090163 
%\item \cite{SVM_MPC} : Data-driven model predictive control for power demand management and fast demand response of commercial buildings using support vector regression : https://link.springer.com/article/10.1007/s12273-021-0811-x. SVR-based MPC solved via genetic algorithm. 
%\end{itemize}

%Data-driven approach. Problem of tractability. \cite{WANG_2023} : Comparison of reinforcement learning and model predictive control for building energy system optimization. The MPC controller is based on a reduced-order thermal resistance-capacity network model. Results showed that the MPC controller is superior to the RL and baseline controller on scenarios on the virtual test bed (Modelica).  \cite{DRL_2022} Approach based on deep reinforcement learning.  . Non-optimization based data-driven method remain impletmented in pratice due to performance, scalability and robustness : \cite{DPC_2018} : Data-driven predictive control based on random forests. Random Forest algorithm do not provide a closed form expression and thus cannot be used for MPC. In \cite{DENG_2023}, \textcolor{red}{(not MPC)} data-driven predictive control : Evaluate effectiveness, robustness and scalability of data-driven predictive control. The experiment was conducted on 78 buildings of the RTEM database and historical data were used to train a deep neural network (DNN) as a building model and was then used to for energy saving. Average energy saving of 65 \% and peak load reduction of 15 \% compared to control. \textcolor{red}{combining conventionnal controller and data-driven modeling}. Limitation of MPC and data-driven : lead to untractability. Many neural-network MPCs and therefore non-convexe approaches were proposed.  Optmization based and data-driven neural-network based method like MPC face the issue of comptutationnal tractability and global optimality : In \cite{BBAI}  an LSTM with attention mechanism based MPC with a genetic algorithm. Non-convex, cannot garantee optimality. \cite{building_RNN} :  model-free and data-driven approach based on a \gls{rnn} to modeling the  and optimization of complex building energy systems with deep neural networks. The MPC is reformulated as an unconstrained optimization problem and then solved via an iterative gradients descent with momentum in order to find the optimal continuous control inputs. Simulation results on an office building showed significant improvement compared to RC controller. \cite{SVM_MPC} 


%To optimize programs involving \glspl{nn}, whether they serve as constraints or objective functions, numerous approaches have been employed within the literature. \textcolor{red}{On continuous problems, both for the convex and non-convex programs}. In the case of convex programs, gradient-based approaches have been preferred since they exploit the problem's convexity and since gradients of a \gls{nn} can be easily computed using backpropagation. In~\cite{chen2018optimal} and~\cite{Amos}, the \gls{nn} objectives are respectively optimized using gradient descent and a custom epigraph cutting plane method. A \gls{dfo} method has also been employed on convex programs. In~\cite{Bünning}, the \gls{nn}-constrained \gls{mpc} is solved using the \gls{dfo} algorithm \texttt{COBYLA}. For the non-convex case, a wide variety of methods have been employed on \gls{nn}-constrained \gls{mpc}, such as an \texttt{SLSQP} algorithm in~\cite{Market_NN_constrained}, the \gls{dfo} algorithm \texttt{BOBYQA} in~\cite{negri2017evaluation}, and a particle swarm optimization a metaheuristic in~\cite{su2022}. Another stream of literature focuses on \gls{milp} reformulation of ReLu-based \gls{nn} as it has the benefits of producing provably optimal solutions~\cite{Anderson_2020,Tsay_2021}. While this approach allows for optimization of mixed integer programs, its main drawback is that it introduces a large number of variables which can lead to intractability in the \gls{mpc} context. On the non-convex problem, mixed-integer approaches predominantly rely on \gls{dfo}, such as a genetic algorithm in~\cite{BBAI}.  % and \gls{dfo}~\cite{liu2017zoopt}.\\

%Also, exact and computational effective reformulation for various \gls{nn} architectures have not yet been developed in the litterature. 
%\textcolor{red}{Justification du choix de method:}
%It should be noted that a gradient-based optimization based method will always outperform \gls{dfo}. Hence, results presented are a lower bound on possible performances of the controller. We choose this method as is it a mature solver. and does not require the exhaustive task of writting the derivative, hence can be readily implementable. In the methods readily available, only \gls{mip} reformulation, some metaheuristics algorithms and some \gls{dfo} algorithms. In this work, we base our approach on the \gls{dfo} mature solver \texttt{NOMAD}. It should be emphasis that a gradient-based approach will always outperform \gls{dfo}, as a results obtained are a lower-bound on the possible performances of the controller. 

%hand, \gls{nn} with ReLU activation are piecewise linear \cite{arora2018understanding}, and therefore non-smooth optimization programs.

%The piecewise linear nature has encourage approaches consisting to reformulate the ReLu-based \gls{nn} as the \gls{mip} reformulation has the benefits of producing provably optimal solutions \cite{Anderson_2020,Tsay_2021}. This approach can approach makes integer optimization variables straightforward. However, it has the downside of introduce a large number of binary variable wich can leads to intractabability in the \gls{mpc} context. Also, these is a lack of exact and computational effective reformulation for various \gls{nn} architectures have not yet been developed in the litterature.
%Other approachs based on metaheuristic such as via genetic algorithm have been applied to solve non-convex mixed-integer \cite{BBAI} . In the methods readily available, only \gls{mip} reformulation, some metaheuristics algorithms and some \gls{dfo} algorithms. In this work, we base our approach on the \gls{dfo} mature solver \texttt{NOMAD}. It should be emphasis that a gradient-based approach will always outperform \gls{dfo}, as a results obtained are a lower-bound on the possible performances of the controller. 



%Other have focused on gradient based method exploting the fact that gradients of \gls{nn} can be easily computed via backpropagation, or bundled entropy method. ReLu-based \gls{nn} are non-smooth function, so gradient descent is not garanteed to converge. Moreover. other approaches where based on \gls{dfo}. It should be emphasised that all approaches were considering continous variables. In this work, we base our approach on \gls{dfo}
%\cite{WANG} : Comparison of reinforcement learning and model predictive control for building energy system optimization. The MPC controller is based on a reduced-order thermal resistance-capacity network model. Results showed that the MPC controller is superior to the RL and baseline controller on scenarios on the virtual test bed (Modelica). 

%\begin{itemize}
%\item Optimization-Based Data-Enabled Modeling Technique for HVAC Systems Components: https://doi.org/10.3390/buildings10090163 
%\item https://doi.org/10.1016/j.engappai.2023.106226
%\item https://doi.org/10.1016/j.enbuild.2017.02.012 
%\end{itemize}


%To optimize programs involving \glspl{nn}, whether they serve as constraints or objective functions, numerous approaches have been employed within the literature. \textcolor{red}{On continuous problems, both for the convex and non-convex programs}. In the case of convex programs, gradient-based approaches have been preferred since they exploit the problem's convexity and since gradients of a \gls{nn} can be easily computed using backpropagation. In~\cite{chen2018optimal} and~\cite{Amos}, the \gls{nn} objectives are respectively optimized using gradient descent and a custom epigraph cutting plane method. A \gls{dfo} method has also been employed on convex programs. In~\cite{Bünning}, the \gls{nn}-constrained \gls{mpc} is solved using the \gls{dfo} algorithm \texttt{COBYLA}. For the non-convex case, a wide variety of methods have been employed on \gls{nn}-constrained \gls{mpc}, such as an \texttt{SLSQP} algorithm in~\cite{Market_NN_constrained}, the \gls{dfo} algorithm \texttt{BOBYQA} in~\cite{negri2017evaluation}, and a particle swarm optimization a metaheuristic in~\cite{su2022}. Another stream of literature focuses on \gls{milp} reformulation of ReLu-based \gls{nn} as it has the benefits of producing provably optimal solutions~\cite{Anderson_2020,Tsay_2021}. While this approach allows for optimization of mixed integer programs, its main drawback is that it introduces a large number of variables which can lead to intractability in the \gls{mpc} context. On the non-convex problem, mixed-integer approaches predominantly rely on \gls{dfo}, such as a genetic algorithm in~\cite{BBAI}.  % and \gls{dfo}~\cite{liu2017zoopt}.\\

%Also, exact and computational effective reformulation for various \gls{nn} architectures have not yet been developed in the litterature. 
%\textcolor{red}{Justification du choix de method:}
%It should be noted that a gradient-based optimization based method will always outperform \gls{dfo}. Hence, results presented are a lower bound on possible performances of the controller. We choose this method as is it a mature solver. and does not require the exhaustive task of writting the derivative, hence can be readily implementable. In the methods readily available, only \gls{mip} reformulation, some metaheuristics algorithms and some \gls{dfo} algorithms. In this work, we base our approach on the \gls{dfo} mature solver \texttt{NOMAD}. It should be emphasis that a gradient-based approach will always outperform \gls{dfo}, as a results obtained are a lower-bound on the possible performances of the controller. 

%hand, \gls{nn} with ReLU activation are piecewise linear \cite{arora2018understanding}, and therefore non-smooth optimization programs.

%The piecewise linear nature has encourage approaches consisting to reformulate the ReLu-based \gls{nn} as the \gls{mip} reformulation has the benefits of producing provably optimal solutions \cite{Anderson_2020,Tsay_2021}. This approach can approach makes integer optimization variables straightforward. However, it has the downside of introduce a large number of binary variable wich can leads to intractabability in the \gls{mpc} context. Also, these is a lack of exact and computational effective reformulation for various \gls{nn} architectures have not yet been developed in the litterature.
%Other approachs based on metaheuristic such as via genetic algorithm have been applied to solve non-convex mixed-integer \cite{BBAI} . In the methods readily available, only \gls{mip} reformulation, some metaheuristics algorithms and some \gls{dfo} algorithms. In this work, we base our approach on the \gls{dfo} mature solver \texttt{NOMAD}. It should be emphasis that a gradient-based approach will always outperform \gls{dfo}, as a results obtained are a lower-bound on the possible performances of the controller. 



%Other have focused on gradient based method exploting the fact that gradients of \gls{nn} can be easily computed via backpropagation, or bundled entropy method. ReLu-based \gls{nn} are non-smooth function, so gradient descent is not garanteed to converge. Moreover. other approaches where based on \gls{dfo}. It should be emphasised that all approaches were considering continous variables. In this work, we base our approach on \gls{dfo}
%\cite{WANG} : Comparison of reinforcement learning and model predictive control for building energy system optimization. The MPC controller is based on a reduced-order thermal resistance-capacity network model. Results showed that the MPC controller is superior to the RL and baseline controller on scenarios on the virtual test bed (Modelica). 

%\begin{itemize}
%\item Optimization-Based Data-Enabled Modeling Technique for HVAC Systems Components: https://doi.org/10.3390/buildings10090163 
%\item https://doi.org/10.1016/j.engappai.2023.106226
%\item https://doi.org/10.1016/j.enbuild.2017.02.012 
%\end{itemize}


%\subsection{Contributions}

%In this work, we design a readily implementable energy management method for small- to medium-sized \glspl{cb} equipped with \gls{rtu}-\gls{hvac}. Our approach is based on a convex \gls{mpc} and uses an \gls{icrnn} to model the thermal dynamics in a data-driven way. Contrarily to previous work \cite{Amos,chen2019, bunning_MPC, BUNNING_2022} in this literature stream, we consider discrete controls to accurately model the operation of most \gls{rtu}-\gls{hvac} \glspl{cb}. Discrete control models promote minimal building upgrades and hence increases its potential for practical implementation. We propose a resolution method based on a \gls{dfo} solver. The convexity of our approach prevents the solver from getting trapped in local minima. Then, we formulate a \gls{dr} strategy where \glspl{cb} can bid flexibility in a real-time market and present case studies in various \gls{dr} program to showcase the full potential of our method. We test our method on a Modelica~\cite{WetterZuoNouiduiPang2014} simulation of 2-zones \gls{cb}, a state-of-the-art numerical simulation.
%\paragraph{Contributions} 

==> Trash/Tikz.tex <==

%Zone separation 
%\begin{tikzpicture}{scale=0.5}
  % Main building rectangle
%  \draw (0,0) rectangle (8,4);
%  \node at (4,2) {};
  
  % Dashed line to separate Zone 1 and Zone 2
%  \draw[dashed] (4,0) -- (4,4);
  
  % Label Zone 1
%  \node at (2,2) {Zone 1};
  
  % Label Zone 2
%  \node at (6,2) {Zone 2};
  
  % RTU 1 for Zone 1
%  \draw (1.25,4) rectangle (2.75,4.5);
%  \node at (2,4.25) {RTU 1};
  
%  % RTU 2 for Zone 2
%  \draw (5.25,4) rectangle (6.75,4.5);
%  \node at (6,4.25) {RTU 2};
%\end{tikzpicture}


==> Trash/accronym.tex <==
\newacronym{rtu}{RTU}{rooftop unit} 
\newacronym{icrnn}{ICRNN}{input convex recurrent neural network}
\newacronym{mpc}{MPC}{model predictive control} 
\newacronym{lstm}{LSTM}{long short-term memory} 
\newacronym{rnn}{RNN}{recurrent neural network} 
\newacronym{nn}{NN}{neural network} 
\newacronym{hvac}{HVAC}{heating ventilation and air conditioning}  
\newacronym{icnn}{ICNN}{Input Convex Neural Network}
\newacronym{ficnn}{FICNN}{Fully Input Convex Neural Network}
\newacronym{picnn}{PICNN}{Partially Input Convex Neural Network}
\newacronym{nem}{NEM}{ustralian National Electricity Market}
\newacronym{fcas}{FCAS}{Frequency control ancillary services} 
\newacronym{dr}{DR}{demand response} 
\newacronym{iso}{ISO}{independent system operator} 
\newacronym{armax}{ARMAX}{Autoregressive-Moving-Average with Exogenous Inputs} 
\newacronym{vns}{VNS}{Variable Neighborhood Search}
\newacronym{mads}{MADS}{Mesh Adaptive Direct Search} 
%\newacronym{dfo}{DFO}{Derivative-Free Optimization} 
\newacronym{oat}{OAT}{outdoor air temperature}
\newacronym{iat}{IAT}{indoor air temperature}
\newacronym{ghi}{GHI}{global horizontal irradiance}
\newacronym{mip}{MIP}{Mixed-Integer Program}
\newacronym{milp}{MIP}{Mixed-Integer Linear Program}

\newglossaryentry{dfo}{
  name={DFO},
  description={Derivative-Free Optimization},
  first={Derivative-Free Optimization (DFO)}
}
